Deep adaptative spectral zoom for improved remote heart rate estimation

Recent advances in remote heart rate measurement, motivated by data-driven approaches, have notably enhanced accuracy. However, these improvements primarily focus on recovering the rPPG signal, overlooking the implicit challenges of estimating the heart rate (HR) from the derived signal. While many methods employ the Fast Fourier Transform (FFT) for HR estimation, the performance of the FFT is inherently affected by a limited frequency resolution. In contrast, the Chirp-Z Transform (CZT), a generalization form of FFT, can refine the spectrum to the narrow-band range of interest for heart rate, providing improved frequential resolution and, consequently, more accurate estimation. This paper presents the advantages of employing the CZT for remote HR estimation and introduces a novel data-driven adaptive CZT estimator. The objective of our proposed model is to tailor the CZT to match the characteristics of each specific dataset sensor, facilitating a more optimal and accurate estimation of HR from the rPPG signal without compromising generalization across diverse datasets. This is achieved through a Sparse Matrix Optimization (SMO). We validate the effectiveness of our model through exhaustive evaluations on three publicly available datasets UCLA-rPPG, PURE, and UBFC-rPPG employing both intra- and cross-database performance metrics. The results reveal outstanding heart rate estimation capabilities, establishing the proposed approach as a robust and versatile estimator for any rPPG method.

==> Experiments/table_sota.tex <==
\begin{table*}[t]
  \caption{Performance evaluation of deep CZT estimator in SOTA approaches.}
  \renewcommand{\arraystretch}{1.35}
  \centering
  \adjustbox{width=0.98\textwidth}{
  \begin{tabular}{c|c|cccc|cccc|cccc}
    \hline
    \multirow{3}{1.35cm}{\centering rPPG Approach} & \multirow{3}{*}{HR Method} &\multicolumn{4}{c|}{Intra-database evaluation} & \multicolumn{8}{c}{Cross-database evaluation} \\ 
    \cline{3-14}
    && \multicolumn{4}{|c}{UCLA-rPPG} & \multicolumn{4}{|c}{PURE} & \multicolumn{4}{|c}{UBFC}\\ 
    \cline{3-14}
    &&MAE$\downarrow$&RMSE$\downarrow$&MAPE$\downarrow$&R$\uparrow$&MAE$\downarrow$&RMSE$\downarrow$&MAPE$\downarrow$&R$\uparrow$&MAE$\downarrow$&RMSE$\downarrow$&MAPE$\downarrow$&R$\uparrow$\\ 
    \hline
    \multirow{3}{*}{{\parbox{0.5cm}{\centering POS \cite{wang2016algorithmic}}}} & 
    FFT& 3.17$\pm$0.50& 4.71$\pm$8.18& 4.40$\pm$0.76& 0.87$\pm$0.07&5.91$\pm$1.27&11.43$\pm$43.33&11.29$\pm$2.59&0.89$\pm$0.06&3.22$\pm$0.87&6.50$\pm$20.36&3.70 $\pm$1.06&0.92$\pm$0.06\\  
    & CZT & 2.62$\pm$0.34& 3.56$\pm$2.67& 3.60$\pm$0.50&0.93$\pm$0.05&4.91$\pm$1.04&9.35$\pm$25.41&9.37$\pm$2.13& 0.93$\pm$0.05& \textbf{3.19$\pm$0.86}&\textbf{6.40 $\pm$20.43}&\textbf{3.67$\pm$1.05}& \textbf{0.92$\pm$0.05}\\
    & Deep CZT & \textbf{2.16$\pm$0.30}&\textbf{3.00$\pm$2.10}&\textbf{2.87$\pm$0.38}& \textbf{0.97$\pm$0.04} & \textbf{3.57$\pm$0.75}& \textbf{6.75$\pm$17.11}&\textbf{6.74$\pm$1.56}&\textbf{0.96$\pm$0.04}& 3.86$\pm$0.84& 6.68$\pm$18.43&4.30 $\pm$1.01& 0.91$\pm$0.07\\
    \hline
    \multirow{3}{*}{{\parbox{0.5cm}{\centering Physnet \cite{Yu2019RemotePS}}}} & 
    FFT&2.27$\pm$0.28&2.99$\pm$1.76&2.96$\pm$0.34&0.98$\pm$0.03& 8.89$\pm$1.68& 15.69$\pm$91.31& 12.80$\pm$2.12& 0.74$\pm$0.09&5.93$\pm$1.52&11.48$\pm$62.86&5.95$\pm$1.46&$0.74\pm$0.11\\
    &CZT&2.26$\pm$0.30&3.10$\pm$2.21&2.91$\pm$0.37&0.98$\pm$0.03& \textbf{7.24$\pm$1.80}&15.62$\pm$105.19&\textbf{8.59$\pm$1.70}&0.77$\pm$0.08&\textbf{5.33$\pm$1.22}&\textbf{9.55$\pm$36.23}&\textbf{5.43$\pm$1.25}&\textbf{0.82$\pm$0.09}\\
    &Deep CZT & \textbf{1.78$\pm$0.24}&\textbf{2.47$\pm$1.59}&\textbf{2.32$\pm$0.30}&\textbf{0.98$\pm$0.03}&8.81$\pm$1.60&\textbf{15.14$\pm$73.43}&12.47$\pm$1.95&\textbf{0.81$\pm$0.08}&5.92$\pm$1.18&9.67$\pm$32.0&6.03$\pm$1.20&0.81$\pm$0.09\\
    \hline
    \multirow{3}{*}{{\parbox{0.5cm}{\centering Efficient-Phys \cite{liu2023efficientphys}}}} & 
    FFT & 2.73$\pm$0.45&4.17$\pm$6.21&3.73$\pm$0.67&0.91$\pm$0.06&7.52$\pm$1.53&13.93$\pm$62.49&12.52$\pm$2.70&0.84$\pm$0.07&4.86$\pm$1.07&8.47$\pm$23.78&5.56$\pm$1.28&0.87$\pm$0.08\\  
    & CZT & 2.13$\pm$0.34&3.17$\pm$3.23&2.76$\pm$0.41& 0.95$\pm$0.04&6.41$\pm$1.51&13.28$\pm$75.77&10.11$\pm$2.64&0.84$\pm$0.07&\textbf{3.37$\pm$0.88}&6.64$\pm$20.29&3.81$\pm$1.06&\textbf{0.92$\pm$0.06}\\
    & Deep CZT & \textbf{1.68$\pm$0.26}&\textbf{2.45$\pm$1.61}&\textbf{2.22$\pm$0.32}&\textbf{0.97$\pm$0.03}&\textbf{5.60$\pm$1.51}&\textbf{12.85$\pm$77.25}&\textbf{6.97$\pm$1.50}&\textbf{0.84$\pm$0.07}&3.41$\pm$0.86&\textbf{6.52$\pm$19.52}&\textbf{3.76$\pm$1.03}&0.91$\pm$0.06\\
    \hline
    \multirow{3}{*}{{\parbox{0.5cm}{\centering TDM \cite{comas2022efficient}}}} & 
    FFT & 2.50$\pm$0.34&3.43$\pm$3.02&3.25$\pm$0.41&0.95$\pm$0.04&4.34$\pm$1.23 & 10.37$\pm$69.21 & 7.32$\pm$2.36 & 0.90$\pm$0.06& 4.83$\pm$0.94 & 7.76$\pm$20.97& 5.40$\pm$1.12& 0.89$\pm$0.07 \\  
    & CZT &2.27$\pm$0.30&3.08$\pm$2.23&2.93$\pm$0.36&\textbf{0.97$\pm$0.03}&3.41$\pm$0.93 & 7.94$\pm$34.08 & 5.84$\pm$1.79 & 0.94$\pm$0.05&4.66$\pm$0.97 & 7.84$\pm$21.21& 5.07$\pm$1.09& 0.88$\pm$0.07 \\
    & Deep CZT & \textbf{1.74$\pm$0.26}&\textbf{2.53$\pm$1.67}&\textbf{2.26$\pm$0.32}&\textbf{0.97$\pm$0.03}&\textbf{3.37$\pm$0.66} & \textbf{6.11$\pm$11.54} & \textbf{5.23$\pm$1.11} & \textbf{0.97$\pm$0.03} &\textbf{4.19$\pm$0.78}& \textbf{6.58$\pm$12.99}& \textbf{4.36$\pm$0.82}& \textbf{0.92$\pm$0.06}\\
    \hline

    
  \end{tabular}
  }
  \label{table:sota_adaptation}
\end{table*}
